A POD approach to identify and control PDEs online through State Dependent Riccati equations

We address the control of Partial Differential equations (PDEs) with unknown parameters. Our objective is to devise an efficient algorithm capable of both identifying and controlling the unknown system. We assume that the desired PDE is observable provided a control input and an initial condition. The method works as follows, given an estimated parameter configuration, we compute the corresponding control using the State-Dependent Riccati Equation (SDRE) approach. Subsequently, after computing the control, we observe the trajectory and estimate a new parameter configuration using Bayesian Linear Regression method. This process iterates until reaching the final time, incorporating a defined stopping criterion for updating the parameter configuration. We also focus on the computational cost of the algorithm, since we deal with high dimensional systems. To enhance the efficiency of the method, indeed, we employ model order reduction through the Proper Orthogonal Decomposition (POD) method. The considered problem's dimension is notably large, and POD provides impressive speedups. Further, a detailed description on the coupling between POD and SDRE is also provided. Finally, numerical examples will show the accurateness of our method across two test cases.

==> latex_table/table_noise_cost_adv.tex <==
\begin{tabular}{llllll}
& Unc & SDRE & RL & RL-POD & POD-ric \\ 
\hline 
Cost Functional & 10.3886 & 2.6136 & 2.7373 & 2.7299 & 3.0603 \\ 
\hline 
\end{tabular}

==> latex_table/table_noise_cost_par.tex <==
\begin{tabular}{llllll}
& Unc & SDRE & RL & RL-POD & POD-ric \\ 
\hline 
Cost Functional & 0.82285 & 0.10924 & 0.11724 & 0.11724 & 0.11724 \\ 
\hline 
\end{tabular}

==> latex_table/table_noise_time_adv.tex <==
\begin{tabular}{lllllll}
& SDRE & RL & POD & POD+offline & POD-ric & POD-ric+offline \\ 
\hline 
CPU time & 202.9404 & 199.8525 & 19.9848 & 71.0679 & 178.8718 & 229.9549 \\ 
\hline 
\end{tabular}

==> latex_table/table_noise_time_par.tex <==
\begin{tabular}{lllllll}
& SDRE & RL & POD & POD+offline & POD-ric & POD-ric+offline \\ 
\hline 
CPU time & 129.7551 & 128.6038 & 2.236 & 29.8731 & 123.5493 & 151.1864 \\ 
\hline 
\end{tabular}
